'Debunk-It-Yourself': Health Professionals' Strategies for Responding to Misinformation on TikTok

Misinformation is "sticky" in nature, requiring a considerable effort to undo its influence. One such effort is debunking or exposing the falsity of information. As an abundance of misinformation is on social media, platforms do bear some debunking responsibility in order to preserve their trustworthiness as information providers. A subject of interpretation, platforms poorly meet this responsibility and allow dangerous health misinformation to influence many of their users. This open route to harm did not sit well with health professional users, who recently decided to take the debunking into their own hands. To study this individual debunking effort - which we call 'Debunk-It-Yourself (DIY)' - we conducted an exploratory survey n=14 health professionals who wage a misinformation counter-influence campaign through videos on TikTok. We focused on two topics, nutrition and mental health, which are the ones most often subjected to misinformation on the platform. Our thematic analysis reveals that the counterinfluence follows a common process of initiation, selection, creation, and "stitching" or duetting a debunking video with a misinformation video. The 'Debunk-It-Yourself' effort was underpinned by three unique aspects: (i) it targets trending misinformation claims perceived to be of direct harm to people's health; (ii) it offers a symmetric response to the misinformation; and (iii) it is strictly based on scientific evidence and claimed clinical experience. Contrasting the 'Debunk-It-Yourself' effort with the one TikTok and other platforms (reluctantly) put in moderation, we offer recommendations for a structured response against the misinformation's influence by the users themselves.

==> sections/04.paradigm.tex <==
% \section{Debunk-it-Yourself Misinformation}
% A gap in response to misinformation on social media, and in particular on TikTok, exists relative to the symmetric, debunking of falsehoods through content, instead of platform affordances or moderation... 

% % Feel free to use the justification statements as an anchor :) 

% % Amy: A couple of thoughts here regarding the viewpoint we are taking. Basically, the literature provides strategies for the Debunking step in Figure 1. However, I don't recall, and need you to verify this for me, that there was nothing found on the Selection or Initiation steps from Figure 1. I think that is the split and what our paper brings to the art.

% Prior art provides recommendations for combating misinformation from a controlled environment/lab setting. We did not find a study that evaluated how misinformation is being combated 'in the wild'. In our 'research in the wild', we bring together a review of how debunkers are organically debunking misinformation on social media, specifically TikTok.

% Existing strategies for combating misinformation start \textit{after} the misinformation has been identified. We did not find a study discussing the selection process for debunking misinformation. In our study, we have compiled the techniques being used at the front end of the misinformation chain to select target videos.

% A future research effort could provide actionable tactics and techniques for moving the debunking effort left in the misinformation food chain that would be easily adoptable by the existing debunking community and moreover, quickly enable more debunkers to participate.

